Model Repair via Symmetry

The symmetry of a Kripke structure $\mathcal{M}$ has been exploited to replace a model check of $\mathcal{M}$ by a model check of the potentially smaller structure $\mathcal{N}$ obtained as the quotient of $\mathcal{M}$ by its symmetry group $G$. We extend previous work to model repair: identify a substructure that satisfies a given temporal logic formula. We show that the substructures of $\mathcal{M}$ that are preserved by $G$ form a lattice that maps to the substructure lattice of $\mathcal{N}$. We also show the existence of a monotone Galois connection between the lattice of substructures of $\mathcal{N}$ and the lattice of substructures of $\mathcal{M}$ that are "maximal" w.r.t. an appropriately defined group action of $G$ on $\mathcal{M}$. These results enable us to repair $\mathcal{N}$ and then to lift the repair to $\mathcal{M}$. We can thus repair symmetric finite-state concurrent programs by repairing the corresponding $\mathcal{N}$, thereby effecting program repair while avoiding state-explosion.

==> extraMaterial.tex <==

%\section{Abstraction and Symmetry}\label{sec:compare}
%There is some similarity between abstraction and symmetry:

%Example of abstracted repairs that fail to lift because of self-loops that are not realized in the original model. Explanation of how such loops are avoided in the group theoretic context. 

%\section{Ideas for future research}
%Factoring the model, i.e., using symmetry on highly symmetric parts of the model but not on other pieces. If all processes are symmetric over a given piece of the model, you could use symmetry locally when checking over that portion. 

%Ring theoretic approach, i.e., endomorphism group. Consider $n$-mutex, Reduce to counting and reduce back...

%\section{Notes from meeting}
%\begin{itemize}
%    \item Generate the quotient.
%    \item Repair the quotient.
%    \item Based off of Section 6 of Symmetry and Model Checking by Emmerson and Sistla. 
%\end{itemize}

